End-to-End QoS for the Open Source Safety-Relevant RISC-V SELENE Platform

This paper presents the end-to-end QoS approach to provide performance guarantees followed in the SELENE platform, a high-performance RISC-V based heterogeneous SoC for safety-related real-time systems. Our QoS approach includes smart interconnect solutions for buses and NoCs, along with multicore interference-aware statistics units to, cooperatively, achieve end-to-end QoS.

==> 2.0.Background.tex <==
\section{State-of-the-Art}

{\color{red}TBD}



==> 5.0.Results.tex <==
\section{Preliminary Results}

{\color{red}TBD}

